Vibrational and Rotational Spectral Data for Possible Interstellar Detection of AlH$_3$OH$_2$, SiH$_3$OH, and SiH$_3$NH$_2$

This work provides the first full set of vibrational and rotational spectral data needed to aid in the detection of AlH$_3$OH$_2$, SiH$_3$OH, and SiH$_3$NH$_2$ in astrophysical or simulated laboratory environments through the use of quantum chemical computations at the CCSD(T)-F12b level of theory employing quartic force fields for the three molecules of interest. Previous work has shown that SiH$_3$OH and SiH$_3$NH$_2$ contain some of the strongest bonds of the most abundant elements in space. AlH$_3$OH$_2$ also contains highly abundant atoms and represents an intermediate along the reaction pathway from H$_2$O and AlH$_3$ to AlH$_2$OH. All three of these molecules are also polar with AlH$_3$OH$_2$ having the largest dipole of 4.58 D and the other two having dipole moments in the 1.10-1.30 D range, large enough to allow for the detection of these molecules in space through rotational spectroscopy. The molecules also have substantial infrared intensities with many of the frequencies being over 90 km mol$^{-1}$ and falling within the currently uncertain 12-17 $\mu$m region of the spectrum. The most intense frequency for AlH$_3$OH$_2$ is $\nu_9$ which has an intensity of 412 km mol$^{-1}$ at 777.0 cm$^{-1}$ (12.87 $\mu$m). SiH$-3$OH has an intensity of 183 km mol$^{-1}$ at 1007.8 cm$^{-1}$ (9.92 $\mu$m) for $\nu_5$, and SiH$_3$NH$_2$ has an intensity of 215 km mol$^{-1}$ at 1000.0 cm$^{-1}$ (10.00 $\mu$m) for $\nu_7$.

==> tables/Geom_AlH3OH2.tex <==
                                   & Units &       Value \\
\hline                            
R$_0$(H$_1$-Al$_2$)                 &  \AA{}  & 1.59197 \\
R$_0$(Al$_2$-O$_3$)                 &  \AA{}  & 2.04014 \\
R$_0$(Al$_2$-H$_4$)                 &  \AA{}  & 1.60154 \\
% R$_0$(Al$_2$-H$_5$)               &  \AA{}  & 1.60154 \\
R$_0$(O$_3$-H$_6$)                  &  \AA{}  & 0.91884 \\
% R$_0$(O$_3$-H$_7$)                &  \AA{}  & 0.91884 \\
$\angle$$_0$(Al$_2$-H$_1$-O$_3$)    &    deg  & 101.834 \\
$\angle$$_0$(Al$_2$-H$_5$-O$_3$)    &    deg  & 96.206 \\
% $\angle$$_0$(Al$_2$-H$_4$-O$_3$)  &    deg  & 96.206 \\
$\angle$$_0$(O$_3$-H$_6$-Al$_2$)    &    deg  & 116.385 \\
% $\angle$$_0$(O$_3$-H$_7$-Al$_2$)  &    deg  & 116.385 \\
\hline                            
R$_e$(H$_1$-Al$_2$)                 &  \AA{}  & 1.58742 \\
R$_e$(Al$_2$-O$_3$)                 &  \AA{}  & 2.02504 \\
R$_e$(Al$_2$-H$_4$)                 &  \AA{}  & 1.59756 \\
% R$_e$(Al$_2$-H$_5$)               &  \AA{}  & 1.59756 \\
R$_e$(O$_3$-H$_6$)                  &  \AA{}  & 0.96189 \\
% R$_e$(O$_3$-H$_7$)                &  \AA{}  & 0.96189 \\
$\angle_e$(Al$_2$-H$_1$-O$_3$)      &    deg  & 102.741 \\
$\angle_e$(Al$_2$-H$_5$-O$_3$)      &    deg  & 95.695 \\
% $\angle_e$(Al$_2$-H$_4$-O$_3$)    &    deg  & 95.695 \\
$\angle_e$(O$_3$-H$_6$-Al$_2$)      &    deg  & 112.678 \\
% $\angle_e$(O$_3$-H$_7$-Al$_2$)    &    deg  & 112.678 \\


==> tables/Geom_SiH3NH2.tex <==
                                 & Units &       Value \\
\hline                          
R$_0$(H$_1$-Si$_2$)               &  \AA{}  & 1.49434 \\
R$_0$(Si$_2$-N$_3$)               &  \AA{}  & 1.72495 \\
R$_0$(Si$_2$-H$_4$)               &  \AA{}  & 1.48713 \\
% R$_0$(Si$_2$-H$_5$)             &  \AA{}  & 1.48713 \\
R$_0$(N$_3$-H$_6$)                &  \AA{}  & 0.98636 \\
% R$_0$(N$_3$-H$_7$)              &  \AA{}  & 0.98636 \\
$\angle_0$(Si$_2$-H$_1$-N$_3$)    &    deg  & 114.848 \\
$\angle_0$(Si$_2$-H$_5$-N$_3$)    &    deg  & 108.286 \\
% $\angle_0$(Si$_2$-H$_4$-N$_3$)  &    deg  & 108.286 \\
$\angle_0$(N$_3$-H$_6$-Si$_2$)    &    deg  & 121.756 \\
% $\angle_0$(N$_3$-H$_7$-Si$_2$)  &    deg  & 121.756 \\
\hline
R$_e$(H$_1$-Si$_2$)               &  \AA{}  & 1.48654 \\
R$_e$(Si$_2$-N$_3$)               &  \AA{}  & 1.72159 \\
R$_e$(Si$_2$-H$_4$)               &  \AA{}  & 1.47930 \\
% R$_e$(Si$_2$-H$_5$)             &  \AA{}  & 1.47930 \\
R$_e$(N$_3$-H$_6$)                &  \AA{}  & 1.00706 \\
% R$_e$(N$_3$-H$_7$)              &  \AA{}  & 1.00706 \\
$\angle_e$(Si$_2$-H$_1$-N$_3$)    &    deg  & 115.666 \\
$\angle_e$(Si$_2$-H$_5$-N$_3$)    &    deg  & 107.725 \\
% $\angle_e$(Si$_2$-H$_4$-N$_3$)  &    deg  & 107.725 \\
$\angle_e$(N$_3$-H$_6$-Si$_2$)    &    deg  & 119.860 \\
% $\angle_e$(N$_3$-H$_7$-Si$_2$)  &    deg  & 119.860 \\


==> tables/Geom_SiH3OH.tex <==
                               & Units &       Value \\
\hline                        
R$_0$(H$_1$-O$_2$)              &  \AA{}  & 0.92024 \\
R$_0$(O$_2$-Si$_3$)             &  \AA{}  & 1.65312 \\
R$_0$(Si$_3$-H$_4$)             &  \AA{}  & 1.48371 \\
R$_0$(Si$_3$-H$_5$)             &  \AA{}  & 1.49070 \\
% R$_0$(Si$_3$-H$_6$)             &  \AA{}  & 1.49070 \\
$\angle_0$(O$_2$-H$_1$-Si$_3$)  &    deg  & 119.969 \\
$\angle_0$(Si$_3$-O$_2$-H$_4$)  &    deg  & 106.489 \\
$\angle_0$(Si$_3$-O$_2$-H$_5$)  &    deg  & 111.282 \\
% $\angle_0$(Si$_3$-O$_2$-H$_6$)  &    deg  & 111.282 \\
\hline
R$_e$(H$_1$-O$_2$)              &  \AA{}  & 0.95631 \\
R$_e$(O$_2$-Si$_3$)             &  \AA{}  & 1.64771 \\
R$_e$(Si$_3$-H$_4$)             &  \AA{}  & 1.47389 \\
R$_e$(Si$_3$-H$_5$)             &  \AA{}  & 1.48160 \\
% R$_e$(Si$_3$-H$_6$)             &  \AA{}  & 1.48160 \\
$\angle_e$(O$_2$-H$_1$-Si$_3$)  &    deg  & 118.225 \\
$\angle_e$(Si$_3$-O$_2$-H$_4$)  &    deg  & 105.768 \\
$\angle_e$(Si$_3$-O$_2$-H$_5$)  &    deg  & 111.547 \\
% $\angle_e$(Si$_3$-O$_2$-H$_6$)  &    deg  & 111.547 \\


==> tables/Vib_AlH3OH2.tex <==
& Description & Harmonic & Anharmonic\\
\hline
$\nu_1$ $(a'')$ &1.001$S_{11}$& 3900.9 (142) & 3715.0\\
$\nu_2$ $(a')$ &1.001$S_{4}$& 3801.2 (62) & 3624.5\\
$\nu_3$ $(a')$ &0.952$S_{1}$+0.049$S_{3}$& 1920.4 (168) & 1854.5\\
$\nu_4$ $(a')$ &0.951$S_{3}$-0.049$S_{1}$ & 1881.9 (194) & 1819.3\\
$\nu_5$ $(a'')$ &1.001$S_{10}$& 1871.5 (367) & 1809.0\\
$\nu_6$ $(a')$ &0.622$S_{8}$+0.386$S_{7}$& 1649.2 (91) & 1607.4\\
$\nu_7$ $(a'')$ &0.555$S_{14}$-0.394$S_{15}$-0.053$S_{13}$& 796.5 (261) & 785.1\\
$\nu_8$ $(a')$ &0.475$S_{9}$-0.270$S_{6}$-0.159$S_{8}$-0.086$S_{5}$& 794.2 (297) & 778.9\\
$\nu_9$ $(a')$ &0.461$S_{6}$+0.349$S_{9}$+0.186$S_{5}$& 777.0 (412) & 775.3\\
$\nu_{10}$ $(a'')$ &0.548$S_{13}$+0.430$S_{12}$& 713.4 (5) & 664.0\\
$\nu_{11}$ $(a')$ &0.540$S_{5}$+0.186$S_{7}$-0.159$S_{6}$-0.092$S_{9}$& 523.4 (153) & 487.9\\
$\nu_{12}$ $(a')$ &0.430$S_{7}$-0.192$S_{5}$-0.176$S_{8}$+0.116$S_{6}$& 386.5 (148) & 319.7\\
$\nu_{13}$ $(a')$ &1.016$S_{2}$& 372.6 (23) & 350.6\\
$\nu_{14}$ $(a'')$ &0.542$S_{12}$-0.369$S_{13}$-0.093$S_{14}$& 366.0 (5) & 364.1\\
$\nu_{15}$ $(a'')$ &0.613$S_{15}$+0.328$S_{14}$& 94.7 (37) & 225.8\\


==> tables/Vib_SiH3NH2.tex <==
                   &                               Description &     Harmonic &               Anharmonic & Experiment$^a$\\
                  
\hline            
$\nu_1$ $(a'')$    &                             1.001$S_{11}$ &  3677.8 (22) &                   3515.3 &          3547 \\
$\nu_2$ $(a')$     &                              1.000$S_{4}$ &  3584.8 (15) &                   3438.7 &          3445 \\
$\nu_3$ $(a'')$    &                             1.001$S_{10}$ & 2258.0 (141) & 2172.2\rdelim\}{3}{-5mm} &               \\
$\nu_4$ $(a')$     &                              0.977$S_{3}$ &  2256.1 (76) &                   2174.5 &     2172      \\
$\nu_5$ $(a')$     &                              0.978$S_{1}$ & 2208.9 (167) &                   2132.5 &               \\
$\nu_6$ $(a')$     &                 0.783$S_{7}$-0.218$S_{8}$ &  1598.0 (29) &                   1563.7 &          1564 \\
$\nu_7$ $(a')$     &    0.517$S_{6}$+0.387$S_{5}$+0.078$S_{9}$ & 1000.0 (215) &  984.7\rdelim\}{3}{-5mm} &          ~996 \\
$\nu_8$ $(a'')$    & 0.546$S_{14}$-0.334$S_{15}$-0.115$S_{12}$ &   997.5 (65) &                    976.0 &          ~983 \\
$\nu_9$ $(a')$     &                 0.903$S_{9}$-0.107$S_{6}$ &  944.4 (103) &                    932.4 &          ~970 \\
$\nu_{10}$ $(a'')$ &               0.623$S_{13}$-0.352$S_{12}$ &   921.1 (40) &                    885.8 &               \\
$\nu_{11}$ $(a')$  &                              0.938$S_{2}$ &   851.0 (49) &                    842.4 &          ~845 \\
$\nu_{12}$ $(a')$  &    0.612$S_{5}$-0.346$S_{6}$-0.072$S_{9}$ &   712.8 (63) &                    699.2 &      ~670$^b$ \\
$\nu_{13}$ $(a'')$ & 0.495$S_{12}$+0.368$S_{13}$+0.152$S_{14}$ &   629.9 (35) &                    608.7 &      ~670$^b$ \\
$\nu_{14}$ $(a')$  &    0.833$S_{8}$+0.197$S_{7}$+0.044$S_{9}$ &  393.4 (153) &                    244.2 &               \\
$\nu_{15}$ $(a'')$ &               0.683$S_{15}$+0.274$S_{14}$ &   177.5 (13) &                 242.8 \\


==> tables/Vib_SiH3OH.tex <==
& Description & Harmonic & Anharmonic\\
\hline
$\nu_1$ $(a')$ & 0.999$S_{1}$& 3919.8 (82) & 3742.9\\
$\nu_2$ $(a')$ &1.000$S_{3}$& 2286.9 (103) & 2202.0\\
$\nu_3$ $(a')$ &1.001$S_{4}$& 2245.5 (87) & 2167.4\\
$\nu_4$ $(a'')$ &1.001$S_{9}$& 2238.3 (162) & 2159.1\\
$\nu_5$ $(a')$ &0.722$S_{7}$+0.192$S_{6}$-0.047$S_{8}$& 1007.8 (183) & 990.6\\
$\nu_6$ $(a')$ &0.865$S_{8}$+0.065$S_{6}$-0.049$S_{5}$& 987.6 (113) & 966.4\\
$\nu_7$ $(a'')$ &0.665$S_{10}$-0.304$S_{12}$& 967.9 (79) & 952.3\\
$\nu_8$ $(a')$ &0.429$S_{2}$+0.341$S_{5}$+0.226$S_{6}$& 911.2 (70) & 889.9\\
$\nu_9$ $(a')$ &0.521$S_{2}$-0.314$S_{5}$-0.094$S_{6}$+0.069$S_{7}$& 850.0 (126) & 810.9\\
$\nu_{10}$ $(a'')$ &0.961$S_{11}$-0.046$S_{12}$& 729.5 (60) & 712.9\\
$\nu_{11}$ $(a')$ &0.422$S_{6}$-0.286$S_{5}$-0.214$S_{7}$-0.077$S_{8}$& 690.1 (58) & 683.3\\
$\nu_{12}$ $(a'')$ &0.651$S_{12}$+0.342$S_{10}$& 196.2 (93) & 181.1\\


==> tables/quart.tex <==
Constant      &   Units &        \alo &       \sin &       \sio \\
\hline       
$A_0$         &     MHz &     56168.1 &    68818.9 &    77174.6 \\
$B_0$         &     MHz &      9274.6 &    12646.5 &    13775.4 \\
$C_0$         &     MHz &      9130.9 &    12224.7 &    13553.9 \\
\hline       
$\Delta_{J}$  &     kHz &      23.495 &     11.122 &     13.574 \\
$\Delta_{K}$  &     kHz &     165.768 &    359.365 &    463.425 \\
$\Delta_{JK}$ &     kHz &      93.777 &    124.706 &    177.170 \\
$\delta_{J}$  &      Hz &     474.202 &    467.870 &    255.285 \\
$\delta_{K}$  &     kHz &  $-$544.657 & $-$307.033 & $-$658.864 \\
$\Phi_{J}$    &     mHz &   $-$91.250 &   $-$2.035 &   $-$2.752 \\
$\Phi_{K}$    &      Hz &      66.334 &     32.968 &     83.512 \\
$\Phi_{JK}$   &      Hz &      24.203 &      6.555 &     23.787 \\
$\Phi_{KJ}$   &      Hz &   $-$84.242 &  $-$28.812 &  $-$87.728 \\
$\phi_{j}$    & $\mu$Hz & $-$1768.830 & $-$418.967 &    613.039 \\
$\phi_{jk}$   &      Hz &    $-$8.133 &   $-$1.303 &   $-$2.708 \\
$\phi_{k}$    &     kHz &       6.367 &      0.951 &      4.257 \\
\hline       
$\mu$         &       D &        4.58 &       1.21 &       1.29 \\
             

